GeoHand: Unlocking Prior Geometry Knowledge for Monocular 3D Hand Reconstruction

Monocular 3D hand reconstruction is intrinsically a geometric problem, yet RGB appearance features alone often struggle to resolve severe ambiguities caused by self-occlusions and hand-object interactions. While introducing depth can explicitly provide spatial cues, raw sensor-captured depth maps are extensively noisy and incomplete, limiting their usefulness for fine-grained hand reconstruction. To bridge this gap, we propose GeoHand, a novel framework that unlocks high-quality geometric priors from a frozen foundational monocular geometry estimator (MoGe2). Recognizing that these priors are oriented toward general scenes, we introduce a map-level GeoAdapter to recalibrate the spatial features, specifically adapting them for detailed hand reconstruction. Furthermore, to systematically integrate these adapted priors without overwhelming intrinsic RGB appearance cues, we employ a gated cross-modal token fusion strategy. Finally, to secure precise local articulation, we design a Keypoint-Queried Iterative Refiner (KQIR) that uses projected joint locations to query geometry-aware image features for spatial correction. By combining global geometric disambiguation with local refinement in a unified pipeline, GeoHand achieves state-of-the-art performance on FreiHAND, DexYCB, and HO3Dv3, especially under severe occlusions and hand-object interactions.

==> Figures/fig_example.tex <==
\begin{figure}[!t]
  \begin{center}
    \includegraphics[width=\linewidth]{Images/teaser.jpg}
  \end{center}
  \caption{\small Figure caption.}
  \label{fig:label}
\end{figure}

==> Tables/tab_example.tex <==
\begin{table}[!t]
  \caption{Sample table title}
  \centering
  \begin{tabular}{lll}
    \toprule
    Name & Description & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal & $\sim$100 \\
    Axon & Output terminal & $\sim$10 \\
    Soma & Cell body & up to $10^6$ \\
    \bottomrule
  \end{tabular}
  \label{tab:table}
\end{table}
